Investigation of cloud cavitating flow in a venturi using Adaptive Mesh Refinement (AMR)

Unsteady cloud cavitating flow is detrimental to the efficiency of hydraulic machinery like pumps and propellers due to the resulting side-effects of vibration, noise and erosion damage. Modelling such a unsteady and highly turbulent flow remains a challenging issue. In this paper, cloud cavitating flow in a venturi is calculated using the Detached Eddy Simulation (DES) model combined with the Merkle model. The Adaptive Mesh Refinement (AMR) method is employed to speed up the calculation and investigate the mechanisms for vortex development in the venturi. The results indicate the velocity gradients and the generalized fluid element strongly influence the formation of vortices throughout a cavitation cycle. In addition, the cavitation-turbulence coupling is investigated on the local scale by comparing with high-fidelity experimental data and using profile stations. While the AMR calculation is able to predict well the time-averaged velocities and turbulence-related aspects near the throat, it displays discrepancies further downstream owing to a coarser grid refinement downstream and under-performs compared to a traditional grid simulation . Additionally, the AMR calculations is unable to reproduce the cavity width as observed in the experiments. Therefore, while AMR promises to speed the process significantly by refining grid only in regions of interest, it is comparatively in line with a traditional calculation for cavitating flows. Thus, this study intends to provide a reference to employing AMR as a tool to speed up calculations and be able to simulate turbulence-cavitation interactions accurately.

==> sn-article-revised <==
%% BioMed_Central_Bib_Style_v1.01

\begin{thebibliography}{37}
% BibTex style file: bmc-mathphys.bst (version 2.1), 2014-07-24
\ifx \bisbn   \undefined \def \bisbn  #1{ISBN #1}\fi
\ifx \binits  \undefined \def \binits#1{#1}\fi
\ifx \bauthor  \undefined \def \bauthor#1{#1}\fi
\ifx \batitle  \undefined \def \batitle#1{#1}\fi
\ifx \bjtitle  \undefined \def \bjtitle#1{#1}\fi
\ifx \bvolume  \undefined \def \bvolume#1{\textbf{#1}}\fi
\ifx \byear  \undefined \def \byear#1{#1}\fi
\ifx \bissue  \undefined \def \bissue#1{#1}\fi
\ifx \bfpage  \undefined \def \bfpage#1{#1}\fi
\ifx \blpage  \undefined \def \blpage #1{#1}\fi
\ifx \burl  \undefined \def \burl#1{\textsf{#1}}\fi
\ifx \doiurl  \undefined \def \doiurl#1{\url{https://doi.org/#1}}\fi
\ifx \betal  \undefined \def \betal{\textit{et al.}}\fi
\ifx \binstitute  \undefined \def \binstitute#1{#1}\fi
\ifx \binstitutionaled  \undefined \def \binstitutionaled#1{#1}\fi
\ifx \bctitle  \undefined \def \bctitle#1{#1}\fi
\ifx \beditor  \undefined \def \beditor#1{#1}\fi
\ifx \bpublisher  \undefined \def \bpublisher#1{#1}\fi
\ifx \bbtitle  \undefined \def \bbtitle#1{#1}\fi
\ifx \bedition  \undefined \def \bedition#1{#1}\fi
\ifx \bseriesno  \undefined \def \bseriesno#1{#1}\fi
\ifx \blocation  \undefined \def \blocation#1{#1}\fi
\ifx \bsertitle  \undefined \def \bsertitle#1{#1}\fi
\ifx \bsnm \undefined \def \bsnm#1{#1}\fi
\ifx \bsuffix \undefined \def \bsuffix#1{#1}\fi
\ifx \bparticle \undefined \def \bparticle#1{#1}\fi
\ifx \barticle \undefined \def \barticle#1{#1}\fi
\bibcommenthead
\ifx \bconfdate \undefined \def \bconfdate #1{#1}\fi
\ifx \botherref \undefined \def \botherref #1{#1}\fi
\ifx \url \undefined \def \url#1{\textsf{#1}}\fi
\ifx \bchapter \undefined \def \bchapter#1{#1}\fi
\ifx \bbook \undefined \def \bbook#1{#1}\fi
\ifx \bcomment \undefined \def \bcomment#1{#1}\fi
\ifx \oauthor \undefined \def \oauthor#1{#1}\fi
\ifx \citeauthoryear \undefined \def \citeauthoryear#1{#1}\fi
\ifx \endbibitem  \undefined \def \endbibitem {}\fi
\ifx \bconflocation  \undefined \def \bconflocation#1{#1}\fi
\ifx \arxivurl  \undefined \def \arxivurl#1{\textsf{#1}}\fi
\csname PreBibitemsHook\endcsname

%%% 1
\bibitem[\protect\citeauthoryear{Chi et~al.}{2022}]{chi2022erosion}
\begin{barticle}
\bauthor{\bsnm{Chi}, \binits{P.}},
\bauthor{\bsnm{Shilong}, \binits{Z.}},
\bauthor{\bsnm{Jianhong}, \binits{F.}},
\bauthor{\bsnm{Qinfeng}, \binits{L.}},
\bauthor{\bsnm{Yu}, \binits{S.}},
\bauthor{\bsnm{Hao}, \binits{C.}},
\bauthor{\bsnm{Yuxuan}, \binits{C.}},
\bauthor{\bsnm{Yun}, \binits{Y.}}:
\batitle{Erosion experiments of shale using a cavitation jet}.
\bjtitle{Ocean Engineering}
\bvolume{261},
\bfpage{112115}
(\byear{2022})
\end{barticle}
\endbibitem

%%% 2
\bibitem[\protect\citeauthoryear{Wu et~al.}{2023}]{wu2023structure}
\begin{barticle}
\bauthor{\bsnm{Wu}, \binits{X.-Y.}},
\bauthor{\bsnm{Zhang}, \binits{Y.-Q.}},
\bauthor{\bsnm{Xu}, \binits{Z.-Q.}},
\bauthor{\bsnm{Zhao}, \binits{S.}},
\bauthor{\bsnm{Li}, \binits{G.-S.}},
\bauthor{\bsnm{Tian}, \binits{S.-C.}},
\bauthor{\bsnm{Tan}, \binits{Y.-W.}},
\bauthor{\bsnm{Peng}, \binits{K.-W.}}:
\batitle{Structure optimization of the organ-pipe cavitating nozzle and its erosion ability test on hydrate-bearing sediments}.
\bjtitle{Petroleum Science}
\bvolume{20}(\bissue{2}),
\bfpage{1104}--\blpage{1118}
(\byear{2023})
\end{barticle}
\endbibitem

%%% 3
\bibitem[\protect\citeauthoryear{Gopalan and Katz}{2000}]{gopalan2000flow}
\begin{barticle}
\bauthor{\bsnm{Gopalan}, \binits{S.}},
\bauthor{\bsnm{Katz}, \binits{J.}}:
\batitle{Flow structure and modeling issues in the closure region of attached cavitation}.
\bjtitle{Physics of fluids}
\bvolume{12}(\bissue{4}),
\bfpage{895}--\blpage{911}
(\byear{2000})
\end{barticle}
\endbibitem

%%% 4
\bibitem[\protect\citeauthoryear{Arabnejad et~al.}{2019}]{arabnejad2019numerical}
\begin{barticle}
\bauthor{\bsnm{Arabnejad}, \binits{M.H.}},
\bauthor{\bsnm{Amini}, \binits{A.}},
\bauthor{\bsnm{Farhat}, \binits{M.}},
\bauthor{\bsnm{Bensow}, \binits{R.E.}}:
\batitle{Numerical and experimental investigation of shedding mechanisms from leading-edge cavitation}.
\bjtitle{International journal of multiphase flow}
\bvolume{119},
\bfpage{123}--\blpage{143}
(\byear{2019})
\end{barticle}
\endbibitem

%%% 5
\bibitem[\protect\citeauthoryear{Ge et~al.}{2022}]{ge2022combined}
\begin{barticle}
\bauthor{\bsnm{Ge}, \binits{M.}},
\bauthor{\bsnm{Sun}, \binits{C.}},
\bauthor{\bsnm{Zhang}, \binits{G.}},
\bauthor{\bsnm{Coutier-Delgosha}, \binits{O.}},
\bauthor{\bsnm{Fan}, \binits{D.}}:
\batitle{Combined suppression effects on hydrodynamic cavitation performance in venturi-type reactor for process intensification}.
\bjtitle{Ultrasonics Sonochemistry}
\bvolume{86},
\bfpage{106035}
(\byear{2022})
\end{barticle}
\endbibitem

%%% 6
\bibitem[\protect\citeauthoryear{Chen et~al.}{2017}]{chen2017large}
\begin{barticle}
\bauthor{\bsnm{Chen}, \binits{Y.}},
\bauthor{\bsnm{Chen}, \binits{X.}},
\bauthor{\bsnm{Li}, \binits{J.}},
\bauthor{\bsnm{Gong}, \binits{Z.}},
\bauthor{\bsnm{Lu}, \binits{C.}}:
\batitle{Large eddy simulation and investigation on the flow structure of the cascading cavitation shedding regime around 3d twisted hydrofoil}.
\bjtitle{Ocean Engineering}
\bvolume{129},
\bfpage{1}--\blpage{19}
(\byear{2017})
\end{barticle}
\endbibitem

%%% 7
\bibitem[\protect\citeauthoryear{Li et~al.}{2016}]{li2016large}
\begin{barticle}
\bauthor{\bsnm{Li}, \binits{L.}},
\bauthor{\bsnm{Li}, \binits{B.}},
\bauthor{\bsnm{Hu}, \binits{Z.}},
\bauthor{\bsnm{Lin}, \binits{Y.}},
\bauthor{\bsnm{Cheung}, \binits{S.C.}}:
\batitle{Large eddy simulation of unsteady shedding behavior in cavitating flows with time-average validation}.
\bjtitle{Ocean Engineering}
\bvolume{125},
\bfpage{1}--\blpage{11}
(\byear{2016})
\end{barticle}
\endbibitem

%%% 8
\bibitem[\protect\citeauthoryear{Liu et~al.}{2023}]{liu2023investigation}
\begin{barticle}
\bauthor{\bsnm{Liu}, \binits{X.-r.}},
\bauthor{\bsnm{Wang}, \binits{T.}},
\bauthor{\bsnm{Zhao}, \binits{X.-y.}},
\bauthor{\bsnm{Chen}, \binits{T.-r.}}:
\batitle{Les investigation of the tip vortex cavitating flow with special emphasis on the interaction between cavitation and vorticity by a modified cavitation model}.
\bjtitle{Journal of Hydrodynamics}
\bvolume{35}(\bissue{3}),
\bfpage{594}--\blpage{606}
(\byear{2023})
\end{barticle}
\endbibitem

%%% 9
\bibitem[\protect\citeauthoryear{Wang et~al.}{2021}]{wang2021euler}
\begin{botherref}
\oauthor{\bsnm{Wang}, \binits{Z.}},
\oauthor{\bsnm{Cheng}, \binits{H.}},
\oauthor{\bsnm{Ji}, \binits{B.}}:
Euler--lagrange study of cavitating turbulent flow around a hydrofoil.
Physics of Fluids
\textbf{33}(11)
(2021)
\end{botherref}
\endbibitem

%%% 10
\bibitem[\protect\citeauthoryear{Tian et~al.}{2022}]{tian2022multiscale}
\begin{botherref}
\oauthor{\bsnm{Tian}, \binits{B.}},
\oauthor{\bsnm{Li}, \binits{L.}},
\oauthor{\bsnm{Meng}, \binits{Y.}},
\oauthor{\bsnm{Huang}, \binits{B.}}:
Multiscale modeling of different cavitating flow patterns around naca66 hydrofoil.
Physics of Fluids
\textbf{34}(10)
(2022)
\end{botherref}
\endbibitem

%%% 11
\bibitem[\protect\citeauthoryear{Ji et~al.}{2024}]{ji2024cavitation}
\begin{barticle}
\bauthor{\bsnm{Ji}, \binits{B.}},
\bauthor{\bsnm{Wang}, \binits{Z.-y.}},
\bauthor{\bsnm{Cheng}, \binits{H.-y.}},
\bauthor{\bsnm{Bensow}, \binits{R.E.}}:
\batitle{Cavitation research with computational fluid dynamics: From euler-euler to euler-lagrange approach}.
\bjtitle{Journal of Hydrodynamics}
\bvolume{36}(\bissue{1}),
\bfpage{1}--\blpage{23}
(\byear{2024})
\end{barticle}
\endbibitem

%%% 12
\bibitem[\protect\citeauthoryear{Luo et~al.}{2012}]{luo2012numerical}
\begin{botherref}
\oauthor{\bsnm{Luo}, \binits{X.}},
\oauthor{\bsnm{Ji}, \binits{B.}},
\oauthor{\bsnm{Peng}, \binits{X.}},
\oauthor{\bsnm{Xu}, \binits{H.}},
\oauthor{\bsnm{Nishi}, \binits{M.}}:
Numerical simulation of cavity shedding from a three-dimensional twisted hydrofoil and induced pressure fluctuation by large-eddy simulation
(2012)
\end{botherref}
\endbibitem

%%% 13
\bibitem[\protect\citeauthoryear{Li et~al.}{2021}]{li2021multiscale}
\begin{botherref}
\oauthor{\bsnm{Li}, \binits{L.}},
\oauthor{\bsnm{Wang}, \binits{Z.}},
\oauthor{\bsnm{Li}, \binits{X.}},
\oauthor{\bsnm{Zhu}, \binits{Z.}}:
Multiscale modeling of tip-leakage cavitating flows by a combined volume of fluid and discrete bubble model.
Physics of Fluids
\textbf{33}(6)
(2021)
\end{botherref}
\endbibitem

%%% 14
\bibitem[\protect\citeauthoryear{Coutier-Delgosha et~al.}{2003}]{coutier2003evaluation}
\begin{barticle}
\bauthor{\bsnm{Coutier-Delgosha}, \binits{O.}},
\bauthor{\bsnm{Fortes-Patella}, \binits{R.}},
\bauthor{\bsnm{Reboud}, \binits{J.-L.}}:
\batitle{Evaluation of the turbulence model influence on the numerical simulations of unsteady cavitation}.
\bjtitle{Journal of Fluids Engineering}
\bvolume{125}(\bissue{1}),
\bfpage{38}--\blpage{45}
(\byear{2003})
\end{barticle}
\endbibitem

%%% 15
\bibitem[\protect\citeauthoryear{Reboud et~al.}{1998}]{reboud1998two}
\begin{bchapter}
\bauthor{\bsnm{Reboud}, \binits{J.-L.}},
\bauthor{\bsnm{Stutz}, \binits{B.}},
\bauthor{\bsnm{Coutier}, \binits{O.}}:
\bctitle{Two phase flow structure of cavitation: experiment and modeling of unsteady effects}.
In: \bbtitle{3rd International Symposium on Cavitation CAV1998, Grenoble, France},
vol. \bseriesno{26}
(\byear{1998})
\end{bchapter}
\endbibitem

%%% 16
\bibitem[\protect\citeauthoryear{Ji et~al.}{2014}]{ji2014numerical}
\begin{barticle}
\bauthor{\bsnm{Ji}, \binits{B.}},
\bauthor{\bsnm{Luo}, \binits{X.}},
\bauthor{\bsnm{Arndt}, \binits{R.E.}},
\bauthor{\bsnm{Wu}, \binits{Y.}}:
\batitle{Numerical simulation of three dimensional cavitation shedding dynamics with special emphasis on cavitation--vortex interaction}.
\bjtitle{Ocean Engineering}
\bvolume{87},
\bfpage{64}--\blpage{77}
(\byear{2014})
\end{barticle}
\endbibitem

%%% 17
\bibitem[\protect\citeauthoryear{Long et~al.}{2017}]{long2017numerical}
\begin{barticle}
\bauthor{\bsnm{Long}, \binits{X.}},
\bauthor{\bsnm{Cheng}, \binits{H.}},
\bauthor{\bsnm{Ji}, \binits{B.}},
\bauthor{\bsnm{Arndt}, \binits{R.E.}}:
\batitle{Numerical investigation of attached cavitation shedding dynamics around the clark-y hydrofoil with the fbdcm and an integral method}.
\bjtitle{Ocean Engineering}
\bvolume{137},
\bfpage{247}--\blpage{261}
(\byear{2017})
\end{barticle}
\endbibitem

%%% 18
\bibitem[\protect\citeauthoryear{Johansen et~al.}{2004}]{johansen2004filter}
\begin{barticle}
\bauthor{\bsnm{Johansen}, \binits{S.T.}},
\bauthor{\bsnm{Wu}, \binits{J.}},
\bauthor{\bsnm{Shyy}, \binits{W.}}:
\batitle{Filter-based unsteady rans computations}.
\bjtitle{International Journal of Heat and fluid flow}
\bvolume{25}(\bissue{1}),
\bfpage{10}--\blpage{21}
(\byear{2004})
\end{barticle}
\endbibitem

%%% 19
\bibitem[\protect\citeauthoryear{Sun et~al.}{2019}]{sun2019numerical}
\begin{barticle}
\bauthor{\bsnm{Sun}, \binits{T.}},
\bauthor{\bsnm{Wei}, \binits{Y.}},
\bauthor{\bsnm{Zou}, \binits{L.}},
\bauthor{\bsnm{Jiang}, \binits{Y.}},
\bauthor{\bsnm{Xu}, \binits{C.}},
\bauthor{\bsnm{Zong}, \binits{Z.}}:
\batitle{Numerical investigation on the unsteady cavitation shedding dynamics over a hydrofoil in thermo-sensitive fluid}.
\bjtitle{International Journal of Multiphase Flow}
\bvolume{111},
\bfpage{82}--\blpage{100}
(\byear{2019})
\end{barticle}
\endbibitem

%%% 20
\bibitem[\protect\citeauthoryear{Girimaji}{2006}]{girimaji2006partially}
\begin{botherref}
\oauthor{\bsnm{Girimaji}, \binits{S.S.}}:
Partially-averaged navier-stokes model for turbulence: A reynolds-averaged navier-stokes to direct numerical simulation bridging method
(2006)
\end{botherref}
\endbibitem

%%% 21
\bibitem[\protect\citeauthoryear{Apte et~al.}{2023}]{apte2023numerical}
\begin{botherref}
\oauthor{\bsnm{Apte}, \binits{D.}},
\oauthor{\bsnm{Ge}, \binits{M.}},
\oauthor{\bsnm{Coutier-Delgosha}, \binits{O.}}:
Numerical investigation of a cavitating nozzle for jetting and rock erosion based on different turbulence models.
Geoenergy Science and Engineering,
212300
(2023)
\end{botherref}
\endbibitem

%%% 22
\bibitem[\protect\citeauthoryear{Bai et~al.}{2018}]{bai2018large}
\begin{barticle}
\bauthor{\bsnm{Bai}, \binits{X.-r.}},
\bauthor{\bsnm{Cheng}, \binits{H.-y.}},
\bauthor{\bsnm{Ji}, \binits{B.}},
\bauthor{\bsnm{Long}, \binits{X.-p.}}:
\batitle{Large eddy simulation of tip leakage cavitating flow focusing on cavitation-vortex interaction with cartesian cut-cell mesh method}.
\bjtitle{Journal of Hydrodynamics}
\bvolume{30}(\bissue{4}),
\bfpage{750}--\blpage{753}
(\byear{2018})
\end{barticle}
\endbibitem

%%% 23
\bibitem[\protect\citeauthoryear{Cheng et~al.}{2020}]{cheng2020large}
\begin{barticle}
\bauthor{\bsnm{Cheng}, \binits{H.}},
\bauthor{\bsnm{Bai}, \binits{X.}},
\bauthor{\bsnm{Long}, \binits{X.}},
\bauthor{\bsnm{Ji}, \binits{B.}},
\bauthor{\bsnm{Peng}, \binits{X.}},
\bauthor{\bsnm{Farhat}, \binits{M.}}:
\batitle{Large eddy simulation of the tip-leakage cavitating flow with an insight on how cavitation influences vorticity and turbulence}.
\bjtitle{Applied Mathematical Modelling}
\bvolume{77},
\bfpage{788}--\blpage{809}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 24
\bibitem[\protect\citeauthoryear{Berger and Colella}{1989}]{berger1989local}
\begin{barticle}
\bauthor{\bsnm{Berger}, \binits{M.J.}},
\bauthor{\bsnm{Colella}, \binits{P.}}:
\batitle{Local adaptive mesh refinement for shock hydrodynamics}.
\bjtitle{Journal of computational Physics}
\bvolume{82}(\bissue{1}),
\bfpage{64}--\blpage{84}
(\byear{1989})
\end{barticle}
\endbibitem

%%% 25
\bibitem[\protect\citeauthoryear{Fuster et~al.}{2009}]{fuster2009simulation}
\begin{barticle}
\bauthor{\bsnm{Fuster}, \binits{D.}},
\bauthor{\bsnm{Bagu{\'e}}, \binits{A.}},
\bauthor{\bsnm{Boeck}, \binits{T.}},
\bauthor{\bsnm{Le~Moyne}, \binits{L.}},
\bauthor{\bsnm{Leboissetier}, \binits{A.}},
\bauthor{\bsnm{Popinet}, \binits{S.}},
\bauthor{\bsnm{Ray}, \binits{P.}},
\bauthor{\bsnm{Scardovelli}, \binits{R.}},
\bauthor{\bsnm{Zaleski}, \binits{S.}}:
\batitle{Simulation of primary atomization with an octree adaptive mesh refinement and vof method}.
\bjtitle{International Journal of Multiphase Flow}
\bvolume{35}(\bissue{6}),
\bfpage{550}--\blpage{565}
(\byear{2009})
\end{barticle}
\endbibitem

%%% 26
\bibitem[\protect\citeauthoryear{Zhang et~al.}{2018}]{zhang2018coalescence}
\begin{barticle}
\bauthor{\bsnm{Zhang}, \binits{Y.}},
\bauthor{\bsnm{Chen}, \binits{K.}},
\bauthor{\bsnm{You}, \binits{Y.}},
\bauthor{\bsnm{Ren}, \binits{W.}}:
\batitle{Coalescence of two initially spherical bubbles: Dual effect of liquid viscosity}.
\bjtitle{International Journal of Heat and Fluid Flow}
\bvolume{72},
\bfpage{61}--\blpage{72}
(\byear{2018})
\end{barticle}
\endbibitem

%%% 27
\bibitem[\protect\citeauthoryear{Li et~al.}{2020}]{li2020large}
\begin{barticle}
\bauthor{\bsnm{Li}, \binits{L.-m.}},
\bauthor{\bsnm{Hu}, \binits{D.-q.}},
\bauthor{\bsnm{Liu}, \binits{Y.-c.}},
\bauthor{\bsnm{Wang}, \binits{B.-t.}},
\bauthor{\bsnm{Shi}, \binits{C.}},
\bauthor{\bsnm{Shi}, \binits{J.-j.}},
\bauthor{\bsnm{Xu}, \binits{C.}}:
\batitle{Large eddy simulation of cavitating flows with dynamic adaptive mesh refinement using openfoam}.
\bjtitle{Journal of Hydrodynamics}
\bvolume{32},
\bfpage{398}--\blpage{409}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 28
\bibitem[\protect\citeauthoryear{Wang et~al.}{2020}]{wang2020numerical}
\begin{barticle}
\bauthor{\bsnm{Wang}, \binits{Z.}},
\bauthor{\bsnm{Li}, \binits{L.}},
\bauthor{\bsnm{Cheng}, \binits{H.}},
\bauthor{\bsnm{Ji}, \binits{B.}}:
\batitle{Numerical investigation of unsteady cloud cavitating flow around the clark-y hydrofoil with adaptive mesh refinement using openfoam}.
\bjtitle{Ocean Engineering}
\bvolume{206},
\bfpage{107349}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 29
\bibitem[\protect\citeauthoryear{Weller et~al.}{1998}]{Weller1998}
\begin{barticle}
\bauthor{\bsnm{Weller}, \binits{H.G.}},
\bauthor{\bsnm{Tabor}, \binits{G.}},
\bauthor{\bsnm{Jasak}, \binits{H.}},
\bauthor{\bsnm{Fureby}, \binits{C.}}:
\batitle{A tensorial approach to computational continuum mechanics using object orientated techniques}.
\bjtitle{Computers in Physics}
\bvolume{12},
\bfpage{620}--\blpage{631}
(\byear{1998})
\end{barticle}
\endbibitem

%%% 30
\bibitem[\protect\citeauthoryear{Mitchell}{2007}]{mitchell2007refinement}
\begin{barticle}
\bauthor{\bsnm{Mitchell}, \binits{W.F.}}:
\batitle{A refinement-tree based partitioning method for dynamic load balancing with adaptively refined grids}.
\bjtitle{Journal of Parallel and Distributed Computing}
\bvolume{67}(\bissue{4}),
\bfpage{417}--\blpage{429}
(\byear{2007})
\end{barticle}
\endbibitem

%%% 31
\bibitem[\protect\citeauthoryear{Merkle}{1998}]{merkle1998computational}
\begin{bchapter}
\bauthor{\bsnm{Merkle}, \binits{C.L.}}:
\bctitle{Computational modelling of the dynamics of sheet cavitation}.
In: \bbtitle{Proc. of the 3rd Int. Symp. on Cavitation, Grenoble, France, 1998}
(\byear{1998})
\end{bchapter}
\endbibitem

%%% 32
\bibitem[\protect\citeauthoryear{Travin et~al.}{2002}]{travin2002physical}
\begin{bchapter}
\bauthor{\bsnm{Travin}, \binits{A.}},
\bauthor{\bsnm{Shur}, \binits{M.}},
\bauthor{\bsnm{Strelets}, \binits{M.}},
\bauthor{\bsnm{Spalart}, \binits{P.}}:
\bctitle{Physical and numerical upgrades in the detached-eddy simulation of complex turbulent flows}.
In: \bbtitle{Advances in LES of Complex Flows: Proceedings of the Euromech Colloquium 412, Held in Munich, Germany 4--6 October 2000},
pp. \bfpage{239}--\blpage{254}
(\byear{2002}).
\bcomment{Springer}
\end{bchapter}
\endbibitem

%%% 33
\bibitem[\protect\citeauthoryear{Dehkordi et~al.}{2017}]{dehkordi2017cfd}
\begin{barticle}
\bauthor{\bsnm{Dehkordi}, \binits{P.B.}},
\bauthor{\bsnm{Colombo}, \binits{L.P.M.}},
\bauthor{\bsnm{Guilizzoni}, \binits{M.}},
\bauthor{\bsnm{Sotgia}, \binits{G.}}:
\batitle{Cfd simulation with experimental validation of oil-water core-annular flows through venturi and nozzle flow meters}.
\bjtitle{Journal of Petroleum science and Engineering}
\bvolume{149},
\bfpage{540}--\blpage{552}
(\byear{2017})
\end{barticle}
\endbibitem

%%% 34
\bibitem[\protect\citeauthoryear{Ge et~al.}{2021}]{ge2021cavitation}
\begin{barticle}
\bauthor{\bsnm{Ge}, \binits{M.}},
\bauthor{\bsnm{Petkov{\v{s}}ek}, \binits{M.}},
\bauthor{\bsnm{Zhang}, \binits{G.}},
\bauthor{\bsnm{Jacobs}, \binits{D.}},
\bauthor{\bsnm{Coutier-Delgosha}, \binits{O.}}:
\batitle{Cavitation dynamics and thermodynamic effects at elevated temperatures in a small venturi channel}.
\bjtitle{International Journal of Heat and Mass Transfer}
\bvolume{170},
\bfpage{120970}
(\byear{2021})
\end{barticle}
\endbibitem

%%% 35
\bibitem[\protect\citeauthoryear{Apte et~al.}{2024}]{apte2024numerical}
\begin{botherref}
\oauthor{\bsnm{Apte}, \binits{D.}},
\oauthor{\bsnm{Ge}, \binits{M.}},
\oauthor{\bsnm{Coutier-Delgosha}, \binits{O.}}:
Numerical investigation of three-dimensional effects of cavitating flow in a venturi-type hydrodynamic cavitation reactor.
arXiv preprint arXiv:2405.00831
(2024)
\end{botherref}
\endbibitem

%%% 36
\bibitem[\protect\citeauthoryear{Dittakavi et~al.}{2010}]{dittakavi2010large}
\begin{botherref}
\oauthor{\bsnm{Dittakavi}, \binits{N.}},
\oauthor{\bsnm{Chunekar}, \binits{A.}},
\oauthor{\bsnm{Frankel}, \binits{S.}}:
Large eddy simulation of turbulent-cavitation interactions in a venturi nozzle.
Journal of Fluids Engineering
\textbf{132}(12)
(2010)
\end{botherref}
\endbibitem

%%% 37
\bibitem[\protect\citeauthoryear{Laberteaux and Ceccio}{2001}]{laberteaux2001partial}
\begin{barticle}
\bauthor{\bsnm{Laberteaux}, \binits{K.}},
\bauthor{\bsnm{Ceccio}, \binits{S.}}:
\batitle{Partial cavity flows. part 1. cavities forming on models without spanwise variation}.
\bjtitle{Journal of Fluid Mechanics}
\bvolume{431},
\bfpage{1}--\blpage{41}
(\byear{2001})
\end{barticle}
\endbibitem

\end{thebibliography}

